Compiling Combinatorial Genetic Circuits with Semantic Inference

A central strategy of synthetic biology is to understand the basic processes of living creatures through engineering organisms using the same building blocks. Biological machines described in terms of parts can be studied by computer simulation in any of several languages or robotically assembled in vitro. In this paper we present a language, the Genetic Circuit Description Language (GCDL) and a compiler, the Genetic Circuit Compiler (GCC). This language describes genetic circuits at a level of granularity appropriate both for automated assembly in the laboratory and deriving simulation code. The GCDL follows Semantic Web practice and the compiler makes novel use of the logical inference facilities that are therefore available. We present the GCDL and compiler structure as a study of a tool for generating $\kappa$-language simulations from semantic descriptions of genetic circuits.

==> endmatter.tex <==
\section{The Genetic Circuit Compiler Language}
\label{sec:gcc-vocabulary}
\lstinputlisting[language=turtle]{composition.ttl}
\clearpage
\section{Additional Inference Rules for GCC}
\lstinputlisting[language=turtle]{composition.n3}

\acrodef{GCDL}[GCDL]{Genetic Circuit Description Language}
\acrodef{GCC}[GCC]{Genetic Circuit Compiler}
\acrodef{RDF}[RDF]{Resource Description Framework}
\acrodef{SW}[SemWeb]{Semantic Web}
\acrodef{BNGL}[BNGL]{BioNetGen Language}
\acrodef{SBOL}[SBOL]{Synthetic Biology Open Language}
\acrodef{URI}[URI]{Universal Resource Identifier}
\acrodef{KBBF}[KBBF]{Kappa BioBricks Framework}
\acrodef{RBMO}[RBMO]{Rule-Based Model Ontology}
\acrodef{SKOS}[SKOS]{Simple Knowledge Organization System}

